How to Quantify Polarization in Models of Opinion Dynamics

It is widely believed that society is becoming increasingly polarized around important issues, a dynamic that does not align with common mathematical models of opinion formation in social networks. In particular, measures of polarization based on opinion variance are known to decrease over time in frameworks such as the popular DeGroot model. Complementing recent work that seeks to resolve this apparent inconsistency by modifying opinion models, we instead resolve the inconsistency by proposing changes to how polarization is quantified. We present a natural class of group-based polarization measures that capture the extent to which opinions are clustered into distinct groups. Using theoretical arguments and empirical evidence, we show that these group-based measures display interesting, non-monotonic dynamics, even in the simple DeGroot model. In particular, for many natural social networks, group-based metrics can increase over time, and thereby correctly capture perceptions of increasing polarization. Our results build on work by DeMarzo et al., who introduced a group-based polarization metric based on ideological alignment. We show that a central tool from that work, a limit analysis of individual opinions under the DeGroot model, can be extended to the dynamics of other group-based polarization measures, including established statistical measures like bimodality. We also consider local measures of polarization that operationalize how polarization is perceived in a network setting. In conjunction with evidence from prior work that group-based measures better align with real-world perceptions of polarization, our work provides formal support for the use of these measures in place of variance-based polarization in future studies of opinion dynamics.

==> files/oldmiscellaneous.tex <==
	\begin{itemize}
		\item Thinking on societal polarization has become, well, polarized. One one hand, we constantly hear about the dangers of increasing polarization in politics. Polls indicate that people (all over the world or just US?) feel that society is more polarized than ever. On the other, it has been observed that society has reached remarkable consensus on a number of important issues. 
		
		\item In this work, we provide support for this apparently contradiction. In particular, we reexamine the popular DeGroot model for opinion dynamics in social networks. We prove that, even though this model predicts convergence to \emph{consensus} in the asymptotic limit, standard measures of opinion \emph{bimodality} converge to non-zero constants. In fact, we show both theoretically and empirically that asymptotic bimodality can be quite large in both real and synthetic social networks. Even when opinions are becoming more similar in absolute terms, bimodality may be perceived as polarization, which partially explains the contradictory views above.
		
		\item Moreover, we prove that an even stronger form of bimodality arises when opinions on multiple issues are consider simultaneously. Specifically, we show that \emph{ideological consistency} inevitably arises in essentially any social network. I.e., individuals assort into exactly two groups, where all individuals in each group fall on the same ``side'' of all issues. This surprising result is inline with recent empirical findings in the political and social sciences. 
	\end{itemize}


    \section{Experiments}
\begin{figure}[h]
    \centering
    \includegraphics[scale=1]{graphics/converge.pdf}
    \caption{De Groot's opinion formation process run on a
    large SBM graph with $n=10,000$, $p=100/n$, and $q=50/n$
    for 50 iterations.
    Each initial opinion is evolved separately.
    The starting opinions include an opinion vector
    drawn from the uniform
    distribution from -1 to 1, an opinion vector drawn
    from the normal distribution with mean 0 and standard
    deviation 1, an opinion vector drawn from the Laplace
    distribution with mean 0 and standard deviation 1,
    and an opinion vector where half the entries
    were drawn from the normal distribution with standard deviation .1
    centered at -.5 and half the entries were drawn from
    the normal distribution with standard deviation .1
    centered at .5.
    Despite the different starting vectors, the opinions
    all converge to the same bimodality.}
\end{figure}

\begin{figure}[h]
    \centering
    \includegraphics[scale=1]{graphics/groupthink.pdf}
    \caption{De Groot's opinion formation process run on a
    large SBM graph with $n=10,000$, $p=100/n$, and $q=50/n$
    for 100 iterations.
    All four initial opinions were drawn from a normal
    distribution with mean 0 and standard deviation 1.
    The bitstrings on the left represent the opinions
    across all four issues relative to the mean.
    For example, an opinion is counted for `0100'
    when it is below the mean on the first, third, and fourth
    opinions and above the mean on the second opinion.
    Despite evolving each opinion separately,
    nodes fall into either `0100' or its opposite
    `1011' within 10 iterations.
    Then, after plateauing, abruptly switch to `0000'
    and `1111'. Notice that both sets of opinions are
    opposing..}
\end{figure}

The \emph{Friedkin-Johnsen} (FJ) model is similar to DeGroot's Model but, instead
of averaging with the node's own expressed opinion, averages
with the innate opinion.
Intuitively, FJ opinions are more `stubborn.'
Formally,

\begin{align}\label{eq:updateruleFJ}
	z_i^{(t)} = \frac{s_i + \sum_{j \neq i}
		w_{ij}z_j^{(t-1)}}{d_i + 1}
\end{align}

where $z_i^{(t)}$ is the opinion at iteration $t$, $s_i$ is the innate opinion of node $i$, and $d_i$ is the degree of node $i$ in the graph.


%In this project, we use a random graph model termed the Stochastic Block Model (SBM) to construct a graph representing a social network. The SBM is a common generative model seen in numerous fields, including statistics, theoretical computer science, and machine learning \cite{sbm}. We refer the interested reader to \cite{sbm} for a comprehensive survey of applications of the SBM. 
%
%A SBM graph $G$ has $n$ vertices, divided into several communities.
%The probability that there is an edge between two nodes in the same community
%is $p$ while the probability there is an edge between two nodes
%in different communities is $q$.
%
%Often, we have that $p \geq q$, to model the idea that relationships
%within communities are more likely than relationships between
%communities.
%However, there are some real-world situations where $p \leq q$.
%Consider a patient-doctor network and the way opinions of
%e.g. a vaccine are formed.
%Connections representing conversations about a vaccine
%are most likely between a doctor and a patient and less
%likely between patient and patient or doctor and doctor.
%Such a model is particularly relevant to
%the acceptance of COVID-19 vaccines \cite{hoff2020patient-doctor}. When $p=q$, the SBM is known as an Erdős-Rényi graph.
\subsection{DeGroot's Opinion Formation}
The input to both models is a social network
given by a graph and an innate (starting) opinion for each
node in the graph.
That is, each node $i$ has an innate opinion
$s_i$ and expressed opinion (that changes according
to the respective model) $z_i$
where $s_i, z_i \in [-1, 1]$.

\emph{DeGroot's model} updates a node's opinion with the weighted average of its expressed opinion and its friends opinions. Formally,
\begin{align} \label{degroot_update_rule}
	z_i^{(t)} = \frac{z_i^{(t-1)} + \sum_{j \neq i} w_{ij}z_j^{(t-1)}}{d_i + 1}
\end{align}

where $z_i^{(t)}$ is the opinion of node $i$ at iteration $t$,
$z_i^{(t-1)}$ is the opinion of node $i$ in the previous iteration,
and $d_i$ is the degree of node $i$ in the graph.
\medskip \medskip


\subsection{SBM Analysis}
Note: We can do the following in a simpler fashion by only considering the expected adjacency matrix $\bar{A}$. We can write this matrix as $USU^T+(-p+1)I$ where $U$ is the $2n\times2$ vector consisting of the all 1s vector and the vector of $n$ 1s followed by $n$ -1s and $S$ is the $2 \times 2$ diagonal matrix with $np+nq$ and $np-nq$. 

Consider the expected SBM. We'll roughly follow the analysis in Section 4.3 of Chris's paper. The expected adjacency matrix $A$ has 1's down the diagonal (because de Groot's averages a node's previous opinion), $p$ on the on diagonal blocks and $q$ on the off diagonal blocks. We can then write
$$A + pI - I = U S U^T$$ where $U$ is composed of the normalized all 1's vector and the normalized half-one-half-minus-one vector while $S$ is the diagonal matrix with $np+nq$ and $np-nq$.

Now we write the Laplacian 
$$L=D-A = (np+nq)I+I-(A+pI-I)=(np+nq)I-USU^T=U'S'U'^T$$ where $D$ is the degree matrix of $A$, $S'=\textrm{diag}(0,2nq,np+nq,\ldots,np+nq)$, and $U'$ is an orthonormal basis extending $U$.

To get the DAD matrix, we effectively divide the eigenvalues in $S'$ by $np+nq$ and subtract $D^{-1/2}LD^{-1/2}$ from the identity. We end up with $D^{-1/2}AD^{-1/2}=U'S''U'^T$ where $S=\textrm{diag}(1,(np-nq)/(np+nq),0,\ldots,0)$. So a single iteration of the power method (aka de Groot's) will zero out all components except those of the first two eigenvectors.

Lemma \ref{lemma:second_eig_scaling} has two interesting implications. 

\begin{theorem} \label{thm:degroot_converges}
The DeGroot model of opinion dynamics leads to non-zero bimodality. In the limit, any reasonable measure of opinion bimodality (specifically, that is shift and scale invariant) converges to a fixed constant (usually non-zero) that only depends on the graph $G$. This happens even as polarization goes to 0 and even though different initial opinions result in different bimodalities at time $t=0$.
\end{theorem}

\begin{theorem} \label{thm:degroot_opinions_sorted}
The Degroot model inevitably results in "ideological consistency". Specifically, suppose we run the opinion dynamics for several different issues and record which "side" of the average opinion each individual (node) falls on. E.g., if we have 4 issues, we would assign each node 4 bits, marking if that node is either below or above center on each issue. In the limit at t->infinity, nodes will only be assigned exactly two unique bit strings, and those strings will be opposites of each other. I.e., there will be two groups of individuals which disagree on every issue, but are perfectly aligned on their beliefs internally.
\end{theorem}

\subsection{Expected and Perturbed Second Eigenvector}

In this section, we bound the difference between the second eigenvector of the expected and perturbed adjacency matrices. We show that the bimodality of the second eigenvector is close to the bimodality of its expectation. 

\subsection{Assumptions} \label{subsec:assuptions}
We need to following results and assumptions:

We use Davis-Kahan: (from Chris' paper)

\begin{theorem} \label{davis_kahan}
$(\bar{v_2}^Tv_2)^2 \geq 1 - \epsilon'^2/\min(\lambda_i-\lambda_2)^2$
\end{theorem}

where $i\neq2$, $v_2$ (respectively $\bar{v_2}$) is the second eigenvector of $A$ (resp. $\bar{A}$), $\lambda_i$ is the $i$th eigenvalue of $\bar{A}$, and $||A-\bar{A}||_2\leq\epsilon'$.

We also use the following bound on the expected adjacency matrix $\bar{A}$ vs ts. the perturbed adjacency matrix, also from Chris' paper (TODO: look up citation) $A$: $$||A - \bar{A}||_2 \leq 3 \sqrt{pn} = O(pn)$$

We make the following assumption on $p$: $p \geq max \{\frac{log^4 n}{n}, \frac{n^{1/4}}{n}\}$. 

\subsection{Part 1: Proof of Theorem \ref{thm:degroot_converges}}

We first bound the inner product of $\bar{v_2}$ and $v_2$.

Since the eigenvalues of $\bar{A}$ are $pn +qn-p+1$, $pn-nq-p+1$, and 0, we have, by Theorem \ref{davis_kahan} that:

$$(\bar{v_2}^Tv_2)^2 \geq 1 - \frac{pn}{(pn-nq-p+1)^2} \approx 1-\frac{p}{np-nq}$$

When $p=cq$ for some constant $c$, we have:

$$(\bar{v_2}^Tv_2)^2 \geq 1 - \frac{1}{np}$$

Substituting our assumption on $p$ from Section \ref{subsec:assuptions}, we obtain:

$$(\bar{v_2}^Tv_2)^2 \geq 1-\frac{1}{np} = 1 - \epsilon$$ 
for $\epsilon = O(1/n^{1/4})$. 

If we set $\epsilon' = 2\epsilon - \epsilon^2$, we have that

\begin{align} \label{v2_innerprodbound}
(\bar{v_2}^Tv_2) \geq 1 - \epsilon.
\end{align}

\subsection{Part 2: Bimodality}

We also use a special version of the bimodality coefficient. The bimodality coefficient is $\beta=(\gamma^2+1)/\kappa$ where $\gamma$ is the skewness and $\kappa$ is the kurtosis of our opinion vector. Assuming our vector is not skewed, we have a bimodality coefficient of $1/\kappa$.

Suppose $z$ is our resulting opinion vector after De Groot's, then $$\kappa = E[(z-E[z])^4]/E[(z-E[z])^2]^2.$$ From our power method view, we know $z-E[z]=v_2$ the second eigenvector of $A$. Then $$\beta=1/\kappa=1/n||v_2||_2^4/||v_2||_4^4.$$. We define our bimodality coefficient as:

\begin{align} \label{bimodality_coeff}
    \beta= \frac{||v_2||_2^4}{n||v_2||_4^4}
\end{align}

The bimodality of the expected second eigenvector is 1. We want to argue that the bimodality of the perturbed second eigenvector is close to the bimodality of the expected second eigenvector.

\subsection{Part 3: Proof of Theorem \ref{thm:degroot_converges}}

We now have enough to bound the difference between the second eigenvector of the expected and perturbed adjacency matrices.

We can write: $$||v_2 - \bar{v_2}||_2^2 \leq (v_2^Tv_2) -2(\bar{v_2}^Tv_2) + (\bar{v_2}^T\bar{v_2}) \leq 1 -2(1-\epsilon) + 1$$

giving us

\begin{align} \label{expected_perturbed_v2}
    ||v_2 - \bar{v_2}||_2^2 \leq 2\epsilon
\end{align}

Note that we can assume that $v_2$ is normalized since it is an eigenvector, and we plugged in our bound on $(\bar{v_2}^T\bar{v_2})$ from Equation \ref{v2_innerprodbound}. 

Then we just need to worry about the fourth moment of $v_2$. [This](https://math.stackexchange.com/questions/218046/relations-between-p-norms) article tells us that $$\frac{||v_2||_2}{n^{1/4}} \leq ||v_2||_4 \leq ||v_2||_2$$

We have that, by Equation \ref{expected_perturbed_v2}, that: 

$$||v_2 - \bar{v_2}||_4 \leq ||v_2 - \bar{v_2}||_2 \leq  sqrt{2\epsilon}$$

By triangle inequality, we also have that $$| ||v_2||_4 - ||\bar{v_2}||_4 | \leq ||v_2 - \bar{v_2}||_4 \leq  \sqrt{2\epsilon}$$. By algebra, we can write: $$||v_2||_4 \leq ||\bar{v_2}||_4 + \sqrt{2\epsilon}$$.


Recall that $||\bar{v_2}||_4 = \frac{1}{n^{1/4}}$. Substituting into \ref{bimodality_coeff}, we obtain:

\begin{align} \label{bimodality_coeff}
    \beta= \frac{||v_2||_2^4}{n||v_2||_4^4} \geq \frac{1}{n(\frac{1}{n^{1/4}} + \sqrt{2\epsilon})^4} \approx 1
\end{align}

as desired. 

\section{Extension to FJ Dynamics}\label{sec:theory}

Let $z^* = (L + I)^-1s$ be the final equilibrium opinion vector for the FJ dynamics and let $L = D - A$ be the Laplacian for a graph.

Then, the FJ update rule can be written as follows: $$z_{t} = (D + I)^-1(Az_{t-1} + s)$$

Substituting $L = D - A$, we obtain: $$z_{t} = (D + I)^-1(Az_{t-1} + (D + I - A)(D + I - A)^-1s =  (D + I)^-1(Az_{t-1} + (D + I -A)(L + I)^-1s$$

which simplifies to $$z_{t} =  (D + I)^-1(Az_{t-1} + (D + I)(L + I)^-1s -A(L + I)^-1s.$$

By substitution of $z^*$, we can write: $$z_t = (D + I)^-1A(z_{t-1} -(L + I)^-1s) + (D + I)^-1(D + I)(L + I)^-1s = (D + I)^-1A(z_{t-1} -z^*) + z^*.$$

It follows that $$z_t - z^* = (D + I)^-1A(z_{t-1} -z^*)$$, implying that there is a fixed point iteration in the FJ model as we approach $\lim_{t \rightarrow \infty}z^*$. 

Thus, by the Richardson iteration view: $$z_t - z^* = [(D + I)^-1 A]^t(z_0 -z^*)$$


